MolBind: Multimodal Alignment of Language, Molecules, and Proteins

Recent advancements in biology and chemistry have leveraged multi-modal learning, integrating molecules and their natural language descriptions to enhance drug discovery. However, current pre-training frameworks are limited to two modalities, and designing a unified network to process different modalities (e.g., natural language, 2D molecular graphs, 3D molecular conformations, and 3D proteins) remains challenging due to inherent gaps among them. In this work, we propose MolBind, a framework that trains encoders for multiple modalities through contrastive learning, mapping all modalities to a shared feature space for multi-modal semantic alignment. To facilitate effective pre-training of MolBind on multiple modalities, we also build and collect a high-quality dataset with four modalities, MolBind-M4, including graph-language, conformation-language, graph-conformation, and conformation-protein paired data. MolBind shows superior zero-shot learning performance across a wide range of tasks, demonstrating its strong capability of capturing the underlying semantics of multiple modalities.

==> Body/0-Intro.tex <==
Recent years have witnessed the remarkable success of Large language models (LLMs), especially the extensive applications in various domains in recent years~\cite{openai2022intro,openai2023gpt}. However, LLMs are plagued by significant factuality issues, as highlighted by a number of studies~\cite{chen2023felm,ji2023survey,wang2023survey}. These issues significantly undermine the trustworthiness and reliability of LLMs and
% , and the fact that they operate as black-box systems with limited transparency exacerbates the issue.
leads to recent works to understand these factuality issues from the perspective of the models' internal structures~\citep{zou2023representation,halawi2023overthinking,yuksekgonul2023attention,li2023inferencetime} and the decoding patterns~\citet{chuang2023dola}. Although these studies are intriguing, our understanding of the underlying mechanisms that drive factuality issues remains incomplete. \miao{we need to point out the reason why we think it is incomplete -> poor generalization? limited improvement? far from satisfactory? still a long way to go?}. Furthermore, effectively incorporating these internal patterns into the decoding process poses an unresolved challenge.

Different from previous studies, we contribute to the community by providing a different perspective to understand hallucination generation, i.e., from the view of in-context hidden states. This approach is motivated by an interesting observation: the correct answer to a given prompt typically exhibits a higher activation score to the context tokens, whereas a hallucinating answer tends to be less activated within the context. An illustration of this idea can be found at Figure~\ref{fig:box}. In the left example, it can be observed that the incorrect answer "Minilla" exhibits lower activations in the upper layers (layer 26 to 32\miao{the figure is too small to identify the text clearly}), whereas the correct answer "Rome" demonstrates higher activation levels. However, it is important to note that the final layernorm, \miao{if we explain through the layer norm perspective, I suspect it is not just the last layernorm's effect, all the upper layers may contribute together as the activation level is decreasing for "rome" while increasing for "manila"} which significantly adjusts the data distribution, can potentially amplify the score of false answers. As a result, this step may introduce factual errors. \miao{we need to introduce the activation first; not details but it is high level meaning; how we should understand the activations, what is its definitions.}

To better capture this model behavior, we define this as "contextual sharpness" and use the entropy term to show the level of contextual sharpness. Specifically, if there are smaller and shallow activations for the generated token to its in-context prompt, the entropy will be large, i.e., closer to uniform distribution; while if the generated tokens have many activations(i.e., the generated token is closely associated with many input entities), the entropy will be quite small. We extract the relation between the generated tokens and their in-context hidden states by projecting the inner representations to vocabulary tokens, which is commonly used in early exit~\cite{ram2022you,dar2022analyzing,geva2023dissecting}. Secondly, we utilize the softmax function to create a distribution across the context, enabling us to calculate the entropy. \miao{I think we may no need to introduce too much details here. It adds the difficulty of understanding. Maybe we just introduce the high level idea of entropy. } Our analysis on CounterFact~\cite{kevin2022locate} demonstrates that our proposed entropy is an effective metric for hallucination detection.  



 % This entropy serves as a measure of the uncertainty or unpredictability of the distribution.
% to extract information from the inner representations by mapping hidden states to vocabulary tokens. This allows us to gain insights into the relationship between in-context hidden states and specific words. Secondly, we utilize the softmax function to create a distribution across the context, enabling us to calculate the entropy. This entropy serves as a measure of the uncertainty or unpredictability of the distribution. Finally, we employ the entropy as a penalty term in the decoding process to create a controllable decoding method known as \texttt{Activations Decoding}. By incorporating this penalty, we aim to encourage more reliable and factually accurate outputs.


% We have discovered a notable pattern in the behavior of large language models regarding factuality/hallucination from the perspective of inner representation. 
% In the context of in-context learning, we found that incorrect generations exhibit fewer activations across the context in the intermediate to upper layers. In contrast, accurate and factual generation tends to manifest with a higher number of activation regions along the context words, facilitating knowledge application. 

% These findings align with previous research suggesting that middle layers predominantly engage in knowledge extraction, while the latter layers are more involved in grammar structuring.
% Specifically, LLMs frequently exhibit inconsistencies within the context they generate as illustrated in Figure~\ref{fig:box}, while the true answers often prevail through majority voting across the context. We exhibit the phenomenon at Figure~\ref{fig:box}.\miao{TODO: add more explanation on the figure}

% To evaluate and quantify this pattern of action, we utilize entropy as a measure to capture the signal. Entropy provides a quantification of the degree of activation among the tokens within the given context. Through our analysis, we have discovered that this metric proves to be a valuable indicator for detecting factual errors.
\begin{figure*}
  \centering
  \includegraphics[width=1\textwidth]{figures/histo.001.jpeg}

  \caption{Visualizing the Inconsistency Phenomenon in LLMs: When factual errors arise, there is an abrupt shift in the context. However, the correct answer tokens prevail through majority voting within the context. \teng{Expain this figure more. Example: In the final layer, the highest logits are erroneously assigned to the token "geography" as the false answer, leading to factual errors in the QA task. However, the entropy of logits at the true answer  "history" in the middle and later layers is significantly lower than that of the false answer token "geography". }
  \miao{TODO: change to the version without 'Your Output'. add more annotation to the image}}
  \label{fig:box}
\end{figure*}
% Building upon this insight, we have developed a novel constrained decoding method aimed at mitigating these factual errors. By leveraging the information provided by the entropy measure, our proposed method introduces constraints during the decoding process to encourage more accurate and consistent outputs.

% Our analysis on CounterFact~\cite{kevin2022locate} demonstrates that our proposed entropy is an effective metric for hallucination detection.

Motivated by these findings and to encourage more reliable and factually accurate outputs, we propose a constraint decoding algorithm, termed as \texttt{Activations Decoding} by using the entropy as a penalty term to adjust the next token probability distribution to encourage the low-entropy token (more likely to be factually correct) to be chosen. 
% in the decoding process to create a controllable decoding method known as \texttt{Activations Decoding}. By incorporating this penalty, we aim to encourage more reliable and factually accurate outputs. 
Extensive experiments across 3 models and 4 datasets demonstrate that \texttt{activation decoding } strikes a better balance between being informative and factually accurate, consistently improving the performance of the whole LlaMa-chat families. As for widely used knowledge-seeking Question Answering tasks including TriviaQA~\cite{joshi2017triviaqa}, Natural Questions~\cite{kwiatkowski2019natural} demonstrating the \texttt{activation decoding } could generate more factual answers. This research contributes to a better understanding of the inner factual behavior of large language models and offers a practical strategy to enhance the quality and reliability of their generated content.

% Our work contributes in the following ways:
% Firstly, we introduce the concept of entropy for a generated token across the context as a reliable signal of factuality. This novel approach provides valuable insights into assessing the credibility of generated content.
% Secondly, we apply this metric to effectively tackle both error detection and reduction problems simultaneously. This metric proves to be highly effective in both fields, offering a comprehensive solution to improve the accuracy and reliability of generated outputs.

\begin{figure*}[t]
  \centering
 
  \includegraphics[width=0.85\textwidth]{figures/edit_1.0.pdf}
 \caption{An overall insight of our method.\teng{I have re-plotted Figure 2 using a different style. You can accept it if it meets your preferences and requirements}}

  \label{fig:box}
\end{figure*}

==> Body/1-RelatedWork.tex <==





==> tables/auroc.tex <==
\begin{table}[t!]
\centering
\normalsize
\newcolumntype{L}[1]{>{\raggedleft\arraybackslash}p{#1}}
\newcolumntype{R}[1]{>{\raggedright\arraybackslash}p{#1}}
\newcolumntype{P}[1]{>{\centering\arraybackslash}p{#1}}
\resizebox{0.97 \linewidth}{!}{
        \begin{tabular}
{@{}R{0.28\linewidth}P{0.3\linewidth}P{0.3\linewidth}}
\toprule
\textbf{Method} & \textbf{FS-CFT}& \textbf{Raw-CFT} \\
\midrule
Self\_Eval & 66.83 & 56.67 \\
Logit\_Seq & 70.79 &72.05   \\
Dola & 55.31&56.01   \\
Logit+Dola & 68.96 &72.27  \\
\midrule
Sub & 71.59 &73.21 \\
entropy & 63.96 &55.16   \\
Logit+entropy & \textbf{72.65} & \textbf{74.15} \\
% Logit+Ours\_entropy+Dola & \textbf{}   \\
\midrule
\bottomrule
\end{tabular}}
\caption{AUROC score on FS-CFT and Raw-CFT among different baselines (including joint probability and dola-fixed joint probability. Here we use 27th layer(check Dola paper and add explanations) }
\label{tab:auroc}
\end{table}

==> tables/auroc_sub-rel.tex <==
\begin{table}[t!]
\centering
\normalsize
\newcolumntype{L}[1]{>{\raggedleft\arraybackslash}p{#1}}
\newcolumntype{R}[1]{>{\raggedright\arraybackslash}p{#1}}
\newcolumntype{P}[1]{>{\centering\arraybackslash}p{#1}}
\resizebox{0.97 \linewidth}{!}{
        \begin{tabular}
    {@{}R{0.28\linewidth}P{0.35\linewidth}P{0.35\linewidth}@{}}
\toprule
\textbf{} & \textbf{Positive} & \textbf{Negative}  \\
\midrule
\multicolumn{3}{c}{\textit{Raw-CFT}}\\
Sample Num & 277 & 87  \\
Ratio & 0.81 & 0.24  \\
Ratio* & 0.78 & 0.29  \\
\midrule
\multicolumn{3}{c}{\textit{FS-CFT}}\\
Sample Num & 700 & 324  \\
Ratio & 0.63 & 0.37  \\
Ratio* & 0.64 & 0.32  \\
\midrule
\bottomrule
\end{tabular}}
\caption{The ratio of true answer's first token appearing among the top-scoring tokens in subject embeddings for positive and negative samples. Here, 'ratio' refers to obtaining the subject embedding within the context, while 'ratio*' indicates extracting the subject and obtaining its corresponding embedding.  }
\label{tab:sub-ans}
\end{table}

==> tables/res_gen.tex <==
\begin{table*}[h!]
\centering
\small
\begin{tabular}{lllll}
\toprule
\multirow{2}{*}{\textbf{Model}} & \multicolumn{4}{c}{\textbf{TruthfulQA}}  \\
\cmidrule(lr){2-5}
 & \bf \%Truth $\uparrow$ & \bf \%Info $\uparrow$ & \bf \%Truth$\ast$Info $\uparrow$ & \textbf{\%Reject} $\downarrow$ \\
\midrule
LLaMa2-7B-chat & 62.9 & 92.8 & 55.8 & 12.7  \\
 % + ITI-paper~\citep{li2023inference} &  89.5& 89.1 & 79.7 & 5.9  \\
  + ITI~\citep{li2023inference} &  66.5& 85.9 & 52.5 & 21.6 \\
  + REPE~\citep{li2023inference} &  64.6& 96.1 & 61.2& 8.1\\
  + REPE\_read~\citep{li2023inference} &  64.3& 89.6 & 54.0& 16.6\\
 + Dola & 61.1 & 97.1 & 58.5 & 7.2  \\
 + Consistent & 63.2&95.8& 59.1\up{3.3} & 9.7\down{3.0} \\
 % + Consistent+Dola & 62.3&97.2& \bf{60.0} &\bf{7.2}\\
\midrule
LLaMa2-13B-chat & 66.5 & 91.1 & 57.5 & 13.6  \\
 % + CD~\citep{li2022contrastive} &  &  &  &  &  &  \\
 % + ITI~\citep{li2023inference} &  61.2& 96.4 & 59.0 & 7.2  \\
  + ITI~\citep{li2023inference} &  66.6& 91.1 & 57.8 & 13.5 \\
  + Dola & 68.1 & 91.8 & 60.0 & 13.0   \\
 + ConsisDecode &68.2 & 91.4 & 59.6\up{2.1} & 13.1\down{0.5}  \\
 + Consistent+Dola &68.2  & 93.0 & \bf{61.3} & \bf{11.5}  \\
\midrule
LLaMa2-70B-chat & 68.8 & 78.3 & 47.1& 30.0  \\
 % + CD~\citep{li2022contrastive} &  &  &  &  &  &  \\
  + ITI~\citep{li2023inference} &  68.8& 78.3 & 47.1 & 30.0  \\
 + Dola & 71.8 & 82.5 & 54.3 & 23.0   \\
 + ConsisentDecode &65.7  & 90.0 & \bf{55.7}\up{8.6} & \bf15.7\down{14.3}\\
 + Consisent+Dola &71.4  & 83.8 & 55.2 & 20.9  \\
\bottomrule
\end{tabular}
\vspace{-5pt}
\caption{Open-ended generation results on TruthfulQA, TrivialQA and HotPotQA. Here, We bold the number that has the best performance of each model and benchmark.}
\label{tab:combined}
\vspace{-5pt}
\end{table*}


==> tables/res_gen_QA.tex <==
\begin{table*}[h!]
\centering
\small
\begin{tabular}{llllllll}
\toprule
\multirow{2}{*}{\textbf{Model}} & \multicolumn{2}{c}{\textbf{TrivalQA}}  & \multicolumn{2}{c}{\textbf{HotPotQA}}  & \multicolumn{2}{c}{\textbf{NQ}}\\
\cmidrule(lr){2-8}
% \cmidrule(lr){6-8}
  &  \textbf{Exact Match} & \textbf{F1 score} &  \textbf{Exact Match}  & \textbf{F1 score}&  \textbf{Exact Match}  & \textbf{F1 score}\\
\midrule
LLaMa2-7B-chat  & 44.4&44.3 & 22.3&22.8 &21.8&20.4 \\
 + ITI~\citep{li2023inference} & \bf46.5&\bf46.5 & 22.6&23.2&23.5&\bf21.5 \\
 + Dola &  45.2&45.3 & 20.4&21.3 &22.8&21.2 \\
 % +REPE&52.1&49.4&23.3&21.1 &25.3&21.2\\
 %  +REPE\_read&47.8&47.6&20.7&21.5 &&\\
 + Consistent & 45.0\up{0.6}&44.4\up{0.1} & \bf20.2\up{4.3}&\bf20.8\up{0.9}&\bf24.2\up{2.4}&20.9\up{0.5}\\
 % + Consistent+Dola & - & 23.4&23.1 \\
\midrule
LLaMa2-13B-chat  & 63.0&60.9 &24.9&27.4 &33.1&28.9 \\
 % + CD~\citep{li2022contrastive} &  &  &  &  &  &  \\
 + ITI~\citep{li2023inference}  & 63.0 & 60.9 & 24.8&27.4&33.1&28.9 \\
  + Dola  & 63.2&61.5&24.5&23.2  &34.6&31.2 \\
 + ConsisDecode  & \bf64.4\up{1.4}&\bf62.7\up{1.8}&\bf24.9\up{1.4}&\bf23.3\up{0.7} &\bf35.8\up{2.7}&\bf32.4\up{3.5} \\
 % + Consistent+Dola & &  &  \\
\midrule
LLaMa2-70B-chat  &73.3&68.4  &30.2&25.5 &40.7&34.1 \\
 % + CD~\citep{li2022contrastive} &  &  &  &  &  &  \\
  + ITI~\citep{li2023inference} & 73.4 & 68.5 & 30.2& 25.6&40.7&34.1 \\
 + Dola &  74.1&72.3 & 31.2&29.0&41.9&36.2 \\
 + ConsisentDecode & \bf74.4\up{1.1}&\bf73.2\up{4.8} &\bf30.7\up{1.3}&\bf27.4\up{1.1} &\bf42.3\up{1.6}&\bf37.4\up{3.3} \\
 % + Consisent+Dola & &  &  \\
\bottomrule
\end{tabular}
\vspace{-5pt}
\caption{Open-ended generation results on TruthfulQA, TrivialQA and HotPotQA. Here, We bold the number that has the best performance of each model and benchmark.}
\label{tab:combined}
\vspace{-5pt}
\end{table*}


==> tables/res_gen_QA_indomain.tex <==
\begin{table*}[ht!]
\centering
\small
\begin{tabular}{llllllll}
\toprule
\multirow{2}{*}{\textbf{Model}} & \multicolumn{2}{c}{\textbf{TriviaQA}}  & \multicolumn{2}{c}{\textbf{HotPotQA}}  & \multicolumn{2}{c}{\textbf{NQ}}\\
\cmidrule(lr){2-8}
% \cmidrule(lr){6-8}
  &  \textbf{Exact Match} & \textbf{F1 score} &  \textbf{Exact Match}  & \textbf{F1 score}&  \textbf{Exact Match}  & \textbf{F1 score}\\
\midrule
LLaMa2-7B-chat  & 44.4&44.3 & 19.6&20.1&21.8&20.4 \\
 + ITI~\citep{li2023inference} & 46.5&46.5 & 19.7&19.7&23.5&21.5 \\
 + Dola &  45.2&45.3 & 20.4&21.3 &22.7&21.2 \\
 % 搞完了dola7B了
 % +REPE&52.1&49.4&23.3&21.1 &25.3&21.2\\
  % +REPE\_read&47.8&47.6&20.7&21.5 &&\\
 + Consistent & 46.4\up{2.0}&46.4\up{2.1} & \bf22.5\up{2.9}&\bf21.1\up{1.0}&\bf23.0\up{1.2}&21.4\up{1.0}\\
  + ConsistentDola & 46.5\up{2.1}&46.5\up{2.2} & \bf22.7\up{3.1}&\bf21.0\up{0.9}&\bf23.0\up{1.2}&21.5\up{1.1}\\
 % + Consistent+Dola & - & 23.4&23.1 \\
\midrule
LLaMa2-13B-chat  & 63.0&60.9 &23.8&21.7 &33.1&28.9 \\
 % + CD~\citep{li2022contrastive} &  &  &  &  &  &  \\
 + ITI~\citep{li2023inference}  & 63.0 & 60.9 & 23.8&21.7&33.1&28.9 \\
  + Dola  & 63.2&61.5&24.5&23.2  &34.6&31.2 \\
   % 搞完了dola13B了
 + ConsisDecode  & \bf64.5\up{1.5}&\bf62.8\up{1.9}&\bf25.6\up{1.8}&\bf26.4\up{4.7} &\bf35.9\up{2.8}&\bf32.5\up{3.6} \\
  + ConsisDola  & \bf63.6\up{0.6}&\bf62.6\up{1.7}&\bf25.5\up{1.7}&\bf26.2\up{4.5} &\bf35.0\up{1.9}&\bf32.1\up{3.2} \\
 % + Consistent+Dola & &  &  \\
\midrule
LLaMa2-70B-chat  &73.3&68.4  &30.2&25.5 &40.7&34.1 \\
 % + CD~\citep{li2022contrastive} &  &  &  &  &  &  \\
  + ITI~\citep{li2023inference} & 73.4 & 68.5 & 30.2& 25.6&40.7&34.1 \\
 + Dola &  74.1&72.3 & 31.2&29.0&41.9&36.2 \\
 + ConsisentDecode & \bf74.2\up{0.9}&\bf73.2\up{4.8} &\bf31.6\up{1.4}&\bf30.1\up{4.6} &\bf42.4\up{1.7}&\bf37.8\up{3.7} \\
  + ConsisentDola & \bf74.4\up{1.1}&\bf73.4\up{5.0} &\bf31.2\up{1.0}&\bf30.2\up{4.7} &\bf42.1\up{1.4}&\bf37.6\up{3.5} \\
 % + Consisent+Dola & &  &  \\
\bottomrule
\end{tabular}
\vspace{-5pt}
\caption{Open-ended generation results on TruthfulQA, TrivialQA and HotPotQA. Here, We bold the number that has the best performance of each model and benchmark.}
\label{tab:combined}
\vspace{-5pt}
\end{table*}


==> tables/res_gen_indomain.tex <==
\begin{table*}[ht]
\centering
\small
\begin{tabular}{lllll}
\toprule
\multirow{2}{*}{\textbf{Model}} & \multicolumn{4}{c}{\textbf{TruthfulQA}}  \\
\cmidrule(lr){2-5}
 & \bf \%Truth $\uparrow$ & \bf \%Info $\uparrow$ & \bf \%Truth$\ast$Info $\uparrow$ & \textbf{\%Reject} $\downarrow$ \\
\midrule
LLaMa2-7B-chat & 62.9 & 92.8 & 55.8 & 12.7  \\
 % + ITI-paper~\citep{li2023inference} &  89.5& 89.1 & 79.7 & 5.9  \\
  + ITI~\citep{li2023inference} &  66.5& 85.9 & 52.5 & 21.6 \\
  + REPE~\citep{li2023inference} &  64.6& 96.1 & 61.2& 8.1\\
  + REPE\_read~\citep{li2023inference} &  64.3& 89.6 & 54.0& 16.6\\
 + Dola & 62.8 & 97.2 & 60.2 & 7.3  \\
 + Consistent & 63.2&95.8& 59.1\up{3.3} & 9.7\down{3.0} \\
 + Consistent+Dola & 62.3&97.2& \bf{60.0} &\bf{7.2}\\
\midrule
LLaMa2-13B-chat & 66.5 & 91.1 & 57.5 & 13.6  \\
 % + CD~\citep{li2022contrastive} &  &  &  &  &  &  \\
 % + ITI~\citep{li2023inference} &  61.2& 96.4 & 59.0 & 7.2  \\
  + ITI~\citep{li2023inference} &  66.6& 91.1 & 57.8 & 13.5 \\
  + Dola & 68.1 & 91.8 & 60.0 & 13.0   \\
 + ConsisDecode &64.3 & 98.0& \bf62.3\up{4.8} & 5.5\down{0.5}  \\
 + Consistent+Dola &68.2  & 93.0 & \bf{61.3} & \bf{11.5}  \\
\midrule
LLaMa2-70B-chat & 68.8 & 78.3 & 47.1& 30.0  \\
 % + CD~\citep{li2022contrastive} &  &  &  &  &  &  \\
  + ITI~\citep{li2023inference} &  68.8& 78.3 & 47.1 & 30.0  \\
 + Dola & 71.8 & 82.5 & 54.3 & 23.0   \\
 + ConsisentDecode &65.7  & 90.0 & \bf{55.7}\up{8.6} & \bf15.7\down{14.3}\\
 + Consisent+Dola &71.4  & 83.8 & 55.2 & 20.9  \\
\bottomrule
\end{tabular}
\vspace{-5pt}
\caption{Open-ended generation results on TruthfulQA, TrivialQA and HotPotQA. Here, We bold the number that has the best performance of each model and benchmark.}
\label{tab:combined}
\vspace{-5pt}
\end{table*}


==> tables/res_gen_lama1.tex <==
\begin{table*}[t!]
\centering
\small
\begin{tabular}{lcccccc}
\toprule
\multirow{2}{*}{\textbf{Model}} & \multicolumn{4}{c}{\textbf{TruthfulQA}} & \multicolumn{2}{c}{\textbf{QA}} \\
\cmidrule(lr){2-5}
\cmidrule(lr){6-7}
 & \bf \%Truth $\uparrow$ & \bf \%Info $\uparrow$ & \bf \%Truth$\ast$Info $\uparrow$ & \textbf{\%Reject} $\downarrow$ & \textbf{TrivialQA} & \textbf{HotpotQA} \\
\midrule
LLaMa-7B & 30.4 & 96.3 & 26.9 & 2.9 & 51.5 &  \\
 + ITI~\citep{li2023inference} & 49.1 & - & \bf 43.5 & - & - & - \\
 + Dola & 42.1 & 98.3 & 40.8 & 0.6 &  45.1 & - \\
 + Consistent & 42.7 & 96.9 & 40.3(0.5/24) & 1.2&\bf51.7(0.4/30) & -\\
\midrule
LLaMa-13B & 38.8 & 93.6 & 32.4 & 6.7 & - & - \\
 + CD~\citep{li2022contrastive} & 55.3 & 80.2 & 44.4 & 20.3 & - & - \\
 + Dola & 48.8 & 94.9 & \bf 44.6 & 2.1 & - & - \\
 + Consistent & - & - & - &- & -\\
\midrule
LLaMa-33B & 62.5 & 69.0 & 31.7 & 38.1 & - & - \\
 + CD~\citep{li2022contrastive} & 81.5 & 45.0 & 36.7 & 62.7 & - & - \\
 + Dola & 56.4 & 92.4 & \bf 49.1 & 8.2 & - & -\\
 + Consistent & - & - & - &- & -\\
\midrule
LLaMa-65B & 50.2 & 84.5 & 34.8 & 19.1 & - & - \\
 + CD~\citep{li2022contrastive} & 75.0 & 57.9 & 43.4 & 44.6 & - & -\\
 + Dola & 54.3 & 94.7 & \bf 49.2 & 4.8 & - & - \\
 + Consistent & - & - & - &- & -\\
\bottomrule
\end{tabular}
\vspace{-5pt}
\caption{Open-ended generation results on TruthfulQA, StrategyQA, and GSM8K.}
\label{tab:combined}
\vspace{-15pt}
\end{table*}


==> tables/res_gen_lama2.tex <==
\begin{table*}[h!]
\centering
\small
\begin{tabular}{lllllll}
\toprule
\multirow{2}{*}{\textbf{Model}} & \multicolumn{4}{c}{\textbf{TruthfulQA}} & \multicolumn{2}{c}{\textbf{QA}} \\
\cmidrule(lr){2-5}
\cmidrule(lr){6-7}
 & \bf \%Truth $\uparrow$ & \bf \%Info $\uparrow$ & \bf \%Truth$\ast$Info $\uparrow$ & \textbf{\%Reject} $\downarrow$ & \textbf{TrivalQA} & \textbf{HotPotQA} \\
\midrule
LLaMa2-7B & 40.8 & 91.3 & 32.6 & 8.4 & - & - \\
 + ITI~\citep{li2023inference} & - & - & - & - & - & - \\
 + Dola & 43.0 & \bf95.8 & 39.4 & 2.1 & - & - \\
 + Consistent(0.5/24) & 43.8 \up{3.0}& 90.8 &35.4 \up{2.8} && - & - \\
 + Consistent+Dola&\textbf{44.8} \up{4.0}&94.2&\textbf{40.1} \up{7.5}&2.7\\
\midrule
LLaMa2-13B & 41.9 & 93.4 &35.5& 8.0 & - & - \\
 + CD~\citep{li2022contrastive} &  &  &  &  &  &  \\
  + Dola & 54.0 & 87.4 & 41.9 &12.7 &  &  \\
 + Consistent &42.1 \up{0.2}&94.3&36.5 \up{1.0}&7.0 &  &  \\
 + Consistent+Dola &\textbf{56.1} \up{14.2} &87.0&\textbf{43.8} \up{8.3}&12.6 \\
\midrule
LLaMa2-70B & 66.0&69.5&35.6 &  37.8&   &  \\
 + CD~\citep{li2022contrastive} &  &  &  &  &  &  \\
 + Dola &  60.3& 86.0 &  46.4& 17.4 &  &  \\
  + Consistent & 64.5 &73.8  &38.4q\up{2.8} &32.7  &  &  \\
 + Consistent+Dola & 60.0 & 87.0 &47.1\up{0.7}  &  15.5&  &  \\
\bottomrule
\end{tabular}
\vspace{-5pt}
\caption{Open-ended generation results on TruthfulQA, TrivialQA and HotPotQA.}
\label{tab:combined}
\vspace{-10pt}
\end{table*}


==> tables/res_mc.tex <==
\begin{table*}[ht]
\centering
\small
\begin{tabular}{@{}p{0.09\linewidth}p{0.22\linewidth}p{0.2\linewidth}p{0.2\linewidth}p{0.2\linewidth}@{}}
\toprule
\textbf{Data}   & \textbf{Model} & \textbf{LLaMa2-7B-chat} & \textbf{LLaMa2-13B-chat}  & \textbf{LLaMa2-70B-chat} \\
\midrule
 \multirow{4}{*}{TQA-MC1}& Baseline& \bf 33.5 & \bf35.3 & 37.3  \\
 % &+ ITI~\citep{li2023inference} & 40.4 & 36.2  & 37.6  \\
 &+ Dola~\citep{chuang2023dola}& 31.7 & 33.5  & 20.9  \\
&+ ConsistDecode\_single & 25.5 & 27.3 & 25.2  \\
 &+ ConsistDecode & 33.0 & 34.1 & \bf 38.1\up{0.8}  \\
% &+ ConsistDecode+Dola & 32.4 & 32.6 & 20.9   \\
\midrule
 \multirow{4}{*}{TQA-MC2}& Baseline& 50.6 & 53.3 & 56.3  \\
 % &+ ITI~\citep{li2023inference} & 59.4 & 54.5  & 56.0  \\
 &+ Dola~\citep{chuang2023dola}& 49.6 & \bf53.7  &48.0  \\
&+ ConsistDecode\_single & \textbf{58.5} \up{7.9}& \bf{57.9}\up{4.6} & 54.0  \\
&+ ConsistDecode & \bf51.4 \up{0.8}& 53.5\up{0.2} & \bf57.4\up{1.1}  \\
% &+ ConsistDecode+Dola & 50.3 & 53.0 & 48.1   \\
\midrule
    \multirow{4}{*}{TQA-MC3}& Baseline& 24.4 & 26.6 & 27.9  \\
 % &+ ITI~\citep{li2023inference} & - & -  & -  \\
 &+ Dola~\citep{chuang2023dola}& 23.7 & \bf27.4 & 23.6  \\
% &+ ConsistDecode\_single & \textbf{30.4} \up{6.0}(26) & \bf{31.0(34)}\up{4.4} & 28.7(59)  \\
&+ ConsistDecode & \bf25.2 \up{0.8}& 26.6 & \bf29.2\up{1.3}  \\
% &+ ConsistDecode+Dola & 24.5 & 27.1 & 23.8   \\
% \midrule
%    \multirow{4}{*}{Factor-Wiki}& Baseline& \bf57.2  & \bf62.0 & \bf69.2  \\
%   % &+ ITI~\citep{li2023inference} & -  & - & -  \\
%   &+ Dola~\citep{chuang2023dola}& 57.0  & 60.7- & 68.1  \\
%  &+ ConsistDecode & 57.0 & \bf62.0 & 68.9 \\
% \midrule
%    \multirow{4}{*}{Factor-Expert}& Baseline& 66.5 & 69.1 & 68.2   \\
%   % &+ ITI~\citep{li2023inference} & - & -  & -  \\
%   &+ Dola~\citep{chuang2023dola}& 50.0  & 52.1 & 54.7  \\
%  &+ ConsistDecode & \textbf{66.5}(0.1/32) & \bf{69.5}(0.1/40) & \bf69.5(0.6/68)  \\


\bottomrule
\end{tabular}
\caption{Multiple choices results on TruthfulQA. Here, We bold the number that has the best performance of each model and benchmark.}

\label{tab:tfqa-mc}
\end{table*}

==> tables/res_mc_lama1.tex <==
\begin{table*}[t!]
\centering
\small
\begin{tabular}{llllll}
\toprule
\multirow{2}{*}{\textbf{Model}}&\multicolumn{3}{c}{\textbf{TruthfulQA}} &\multicolumn{2}{c}{\textbf{FACTOR}}\\
\cmidrule(lr){2-4} \cmidrule(lr){5-6}
 & \textbf{MC1} & \textbf{MC2} & \textbf{MC3} & \textbf{Expert} & \textbf{Wiki}   \\ \midrule
LLaMa-7B & 25.6 & 40.6 & 19.2 & 61.0 & 58.6\\
 + ITI~\citep{li2023inference} & 25.9 & - & - & - & - \\ 
 + Dola &  \bf 32.2 & \bf 63.8 &  32.1 & 50.4 & \bf 62.2 \\
 + Consistent-single-28 &   28.5\up{2.9} &  58.5\up{17.9} & \bf 33.2\up{17.0} & - & - \\
 + Consistent &   - &  - & - & \bf 64.8(0.4/30) & 58.8(0.1/24) \\

\midrule
LLaMa-13B & 28.3 & 43.3 & 20.8 & - & 62.6\\
 + CD~\citep{li2022contrastive} & 24.4 & 41.0 & 19.0 & - & 64.4\\
 + Dola &  28.9 & \bf 64.9 & \bf 34.8 & - & \bf 66.2\\
 + Consistent-single-36 &   \bf 30.7\up{2.4} &  55.8\up{12.5} & 32.1\up{11.3} &  &  \\
+ consistent &    &   &  &  &  \\
\midrule
LLaMa-33B & 31.7 & 49.5 & 24.2 & - & 69.5\\
 + CD~\citep{li2022contrastive} & \bf 33.0 & 51.8 & 25.7 & - & \bf 71.3\\
 + Dola & 30.5 & \bf 62.3 & \bf 34.0 &- & 70.3\\
 + Consistent &    &   &  &  &  \\
 + Consistent & - & - & - &- & -\\
\midrule
LLaMa-65B & 30.8 & 46.9 & 22.7 & - & 72.2\\
 + CD~\citep{li2022contrastive} & 29.3 & 47.0 & 21.5 & - & 71.3\\
 + Dola & \bf 31.1 & \bf 64.6 & \bf 34.3 & - & \bf 72.4\\
 + Consistent &    &   &  &  &  \\
 + Consistent & - & - & - &- & -\\
\bottomrule
\end{tabular}
\vspace{-5pt}
\caption{Multiple choices results on the TruthfulQA and FACTOR.}
\label{tab:tfqa-mc}
\end{table*}
\vspace{-5pt}




==> tables/res_mc_lama2.tex <==
\begin{table*}[t!]
\centering
\small
\begin{tabular}{@{}p{0.09\linewidth}p{0.22\linewidth}p{0.2\linewidth}p{0.2\linewidth}p{0.2\linewidth}@{}}
\toprule
\textbf{Data}   & \textbf{Model} & \textbf{LLaMa2-7B} & \textbf{LLaMa2-13B}  & \textbf{LLaMa2-65B} \\
\midrule
 \multirow{4}{*}{TQA-MC1}& Baseline& 28.4 & 29.1 & 37.8 \\
 &+ ITI~\citep{li2023inference} & - & -  & -  \\
 &+ Dola~\citep{chuang2023dola}& 27.5 & 24.2  & 31.0  \\
&+ Consistent & \textbf{29.0} \up{0.6}(0.5/24) & \textbf{30.1}(0.8/36)\up{1.0} & 37.1(1/72)  \\
&+ Consistent+Dola & 28.2 & 24.1 & 31.2(1/72)\\
\midrule
 \multirow{4}{*}{TQA-MC2}& Baseline& 43.4 & 44.3 & 53.6  \\
 &+ ITI~\citep{li2023inference} & - & -  & -  \\
 &+ Dola~\citep{chuang2023dola}& 44.6 & \textbf{47.7}  & 54.9  \\
&+ Consistent & \textbf{46.9} \up{3.5}& {45.2}\up{0.9} & 54.3 \up{0.7} \\
&+ Consistent+Dola &  \textbf{47.3} \up{3.9} & 47.6 & 55.2(1/72) \up{1.6}  \\
\midrule
    \multirow{4}{*}{TQA-MC3}& Baseline& 20.5 & 20.7 & 27.4  \\
 &+ ITI~\citep{li2023inference} & - & -  & -  \\
 &+ Dola~\citep{chuang2023dola}& 20.8 & \textbf{24.7}  & 31.0  \\
&+ Consistent & \textbf{22.1} \up{1.6} & 21.3\up{0.6} & 27.5\up{0.1}  \\
&+ Consistent+Dola & \textbf{22.2} \up{1.7} & 24.6 & \textbf{31.1}(1/72)\up{3.7}   \\
\midrule
\midrule
\bottomrule
\end{tabular}
\caption{Multiple choices results on TruthfulQA and FACTOR.}

\label{tab:tfqa-mc}
\end{table*}

==> tables/truthful-mc.tex <==
\begin{table*}
\centering
\small
\begin{tabular}{@{}p{0.07\linewidth}p{0.04\linewidth}|p{0.22\linewidth}p{0.13\linewidth}p{0.13\linewidth}p{0.13\linewidth}p{0.13\linewidth}@{}}
\toprule
\textbf{Data} &  & \textbf{Model} & \textbf{LLaMa3-7B-chat} & \textbf{LLaMa2-13B-chat} & \textbf{LLaMa2-33B-chat} & \textbf{LLaMa2-65B-chat} \\
\midrule
 \multirow{12}{*}{TQA} &\multirow{4}{*}{MC1}& Baseline& - & - & - & -  \\
 & &+ ITI~\citep{li2023inference} & - & - & - & -  \\
 & &+ Dola~\citep{chuang2023dola}& - & - & - & -  \\
& &+ Ours & - & - & - & -  \\
\cmidrule{3-7}
   &\multirow{4}{*}{MC2}& Baseline& - & - & - & -  \\
 & &+ ITI~\citep{li2023inference} & - & - & - & -  \\
 & &+ Dola~\citep{chuang2023dola}& - & - & - & -  \\
& &+ Ours & - & - & - & -  \\
\cmidrule{3-7}
   &\multirow{4}{*}{MC3}& Baseline& - & - & - & -  \\
 & &+ ITI~\citep{li2023inference} & - & - & - & -  \\
 & &+ Dola~\citep{chuang2023dola}& - & - & - & -  \\
& &+ Ours & - & - & - & -  \\
\midrule
   \multirow{8}{*}{Factor}&\multirow{4}{*}{Wiki}& Baseline& - & - & - & -  \\
 & &+ ITI~\citep{li2023inference} & - & - & - & -  \\
 & &+ Dola~\citep{chuang2023dola}& - & - & - & -  \\
& &+ Ours & - & - & - & -  \\
\cmidrule{3-7}
   &\multirow{4}{*}{Expert}& Baseline& - & - & - & -  \\
 & &+ ITI~\citep{li2023inference} & - & - & - & -  \\
 & &+ Dola~\citep{chuang2023dola}& - & - & - & -  \\
& &+ Ours & - & - & - & -  \\
\midrule
\midrule
   \multirow{4}{*}{TQA}&& Baseline& - & - & - & -  \\
 & &+ ITI~\citep{li2023inference} & - & - & - & -  \\
 & &+ Dola~\citep{chuang2023dola}& - & - & - & -  \\
& &+ Ours & - & - & - & -  \\
\midrule
   \multirow{4}{*}{TrivialQA}&& Baseline& - & - & - & -  \\
 & &+ ITI~\citep{li2023inference} & - & - & - & -  \\
 & &+ Dola~\citep{chuang2023dola}& - & - & - & -  \\
& &+ Ours & - & - & - & -  \\
\midrule
 \multirow{4}{*}{HotpotQA}&& Baseline& - & - & - & -  \\
 & &+ ITI~\citep{li2023inference} & - & - & - & -  \\
 & &+ Dola~\citep{chuang2023dola}& - & - & - & -  \\
& &+ Ours & - & - & - & -  \\
\midrule
\bottomrule
\end{tabular}
\caption{Multiple choices results on TruthfulQA and FACTOR.}
\label{tab:tfqa-mc}
\end{table*}
